CoopNet: Cooperative Convolutional Neural Network for Low-Power MCUs

Fixed-point quantization and binarization are two reduction methods adopted to deploy Convolutional Neural Networks (CNN) on end-nodes powered by low-power micro-controller units (MCUs). While most of the existing works use them as stand-alone optimizations, this work aims at demonstrating there is margin for a joint cooperation that leads to inferential engines with lower latency and higher accuracy. Called CoopNet, the proposed heterogeneous model is conceived, implemented and tested on off-the-shelf MCUs with small on-chip memory and few computational resources. Experimental results conducted on three different CNNs using as test-bench the low-power RISC core of the Cortex-M family by ARM validate the CoopNet proposal by showing substantial improvements w.r.t. designs where quantization and binarization are applied separately.

==> bg_old.tex <==
\begin{figure}[!t]
\centering
    \includegraphics[scale=0.53]{img/simple_cnn.pdf}
    \caption{Structure of a typical CNN. (a) Basic block of a standard Integer CNN; (b) Basic block of a BNN with binarized weights and activations}
    \label{fig:simple_cnn}
\end{figure}

\subsection{Convolutional Neural Networks (CNNs)}
CNNs are a special class of end-to-end trainable models mostly suited for the classification of multi-dimensional spatial inputs, like multi-channel images. They consist of several computational layers chained to form a deep architecture. Existing CNNs mainly differ for their internal topology, namely, how different kinds of hidden layers are sized and connected. It is however possible to recognize a common structure which is made up of two macroblocks (Fig.~\ref{fig:simple_cnn}): {\em Feature Extraction}, where relevant features learned during the training stage are extracted layer-wise using kernel convolutions; {\em Classification}, where the extracted features get classified.

Within the feature extraction block, the most commonly adopted layers are: {\em convolutional} layers (CONV), which perform multidimensional convolutions between the output tensor generated by the previous layer (also called feature map) and local filter tensors; {\em pooling} layers (POOL), e.g. max pooling or average pooling, which reduce the dimension of feature maps; {\em normalization} layers (NORM), that normalize the distribution (mean and standard deviation) of the activation maps; {\em activation} function (ACT), e.g. ReLU or tanh, which introduces non-linearity. The classification block is built upon {\em fully-connected} layers (FC), which implement a geometric separation of the extracted features, and {\em softmax}, that produces a probability distribution over the available classes.
%{\em dropout} layers that help to mitigate over-fitting 

\begin{comment}
Such layers can be grouped in three main regions, each with a specific function: {\em input layers} handle inputs for computational stages, {\em hidden} layers extract relevant features learned during the training stage, {\em output layers} take the extracted features and run the actual classification that brings to the final labeling. Existing CNNs mainly differ for the topology of the feature extraction region and the classification region. The former is built upon different kind of layers arranged following different topology. There might be {\em convolutional} (CONV) layers that perform multidimensional convolutions between the output generated by the previous layer and some local filter, {\em pooling} layers which reduce the dimension of feature maps, {\em dropout} layers that help to mitigate over-fitting. The latter implements a geometric separation of the extracted features and it typically consists of {\em fully-connected} (FC) neural network that computes scores on each feature map.
\end{comment}

\subsection{Fixed-Point Quantization}
While a CNN training is usually run using a 32-bits floating-point representation, recent studies, e.g. \cite{fixquant,hubara2017quantized}, demonstrate that fixed-point integers with lower arithmetic precision are enough for inference. Fixed-point quantization is becoming a consolidated standard when the target hardware are low-power cores with small memory footprint and reduced instruction set (8/16-bit integer).
%This allows reducing the memory footprint and the inference computational cost exploiting a reduced precision, integer-only arithmetic.
%The literature is plenty of fixed-point quantization schemes, e.g. {\em static/dynamic}, {\em linear/non-linear}. 
A detailed review of all the quantization schemes in literature is out of the scope of this work and interested readers may refer to \cite{fixquant,hubara2017quantized,mixp}. This work adopts the $q$-bit fixed-point quantization proposed in \cite{hubara2017quantized}. The convolution run in a CONV layer between the input feature map ${\bf x} \in \mathbb{R}^{c \times w_{in}\times h_{in}}$ and the local weights ${\bf w} \in \mathbb{R}^{c \times kw\times kh} $ is as follows:
\begin{equation}
    \textbf{x} \ast \textbf{w} = 2^{-2(q-1)} \sum_{i \in C} X_i \cdot W_i
\end{equation}
with $C$ as the number of channels. We set $q=8$ for both weights and activations, and $q=16$ for intermediate results accumulation. 

%We exploit that quantization schema for the baseline model {\em INT8} model. {\bf ANDREA: not clear}

\subsection{Binarized Neural Networks}
Several works proposed CNNs with binary weights and/or activations. BinaryConnect \cite{BinCon} represents the ancestor: weights are binarized using \textit{hard sigmoid} function, while activations remain in full-precision to avoid accuracy drop. The Binarized Neural Networks proposed in \cite{BNN} are the first example of fully binary CNN: both weights and activations are binarized via \textit{sign} function. The CONV layers are simplified through bit-wise XNOR and bit-count. This allows to achieve the highest compression ($\sim32\times$), yet with substantial accuracy loss (up to 28.7\%).
The authors of XNOR-Net \cite{xnor} addressed this drawback introducing a new topology where the binary output of each CONV layer is first re-scaled through a full-precision NORM layer. Fig.~\ref{fig:simple_cnn}-b gives a pictorial description of the basic block deployed in the XNOR-Net, where the suffix {\em Bin} highlights binarized layers. 

The mathematical description of a binary convolution is as follows. Given $\textbf{x} \in \mathbb{R}^{c \times w_{in}\times h_{in}}$ as the input feature and $\textbf{w} \in \mathbb{R}^{c \times kw\times kh} $ as the weights, the generated output is approximated as:
\begin{equation}
\textbf{o} =    \textbf{x} \ast \textbf{w} \approx \text{popcount}\;(\textbf{X}\;  \text{xnor}\;  \textbf{W})
\end{equation}
where \textbf{X} = sign(\textit{\,{\bf x}\,}) and \textbf{W} = sign(\textit{\,{\bf w}\,}). 
The activation function is fused with the batch normalization. Given the bias $B$, together with all batch normalization parameters, i.e. variance $\sigma$, mean $\mu$, scale $\gamma$ and shift factors $\beta$, the  result  of  the convolution {\em o} is binarized as follow:
\begin{equation}
    BinACT_{0,1} (o) = \begin{cases}
                \text{1 }  p \geq -\omega/\phi, \text{else } 0 &(\phi > 0 )\\
                 \text{1 }  p \leq -\omega/\phi, \text{else } 0 &(\phi < 0 ) \\
                \end{cases}
\end{equation}
where $\omega= \beta + \gamma/\sigma(B-\mu)$ and $\phi=\gamma/\sigma$.

An efficient processing of XNOR-Net requires data-paths capable of performing bitwise xnor, bit-counter and comparison. These operators can be implemented with specialized units in case of custom hardware \cite{finn}, or through software routines compiled using the instruction-set available on the target general purpose core \cite{rusci2018}.

%(simply referred as BNN hereafter)
\begin{comment}
\begin{equation}
     Th =  \lceil2^{\,q-1}\cdot(p\cdot\frac{\sigma}{\gamma} - 2^{\,q-1} \cdot (B -\mu)+ \beta \cdot \frac{\sigma}{\gamma}\rceil
\end{equation}
\end{comment}

